PointNorm-Net: Self-Supervised Normal Prediction of 3D Point Clouds via Multi-Modal Distribution Estimation

Although supervised deep normal estimators have recently shown impressive results on synthetic benchmarks, their performance deteriorates significantly in real-world scenarios due to the domain gap between synthetic and real data. Building high-quality real training data to boost those supervised methods is not trivial because point-wise annotation of normals for varying-scale real-world 3D scenes is a tedious and expensive task. This paper introduces PointNorm-Net, the first self-supervised deep learning framework to tackle this challenge. The key novelty of PointNorm-Net is a three-stage multi-modal normal distribution estimation paradigm that can be integrated into either deep or traditional optimization-based normal estimation frameworks. Extensive experiments show that our method achieves superior generalization and outperforms state-of-the-art conventional and deep learning approaches across three real-world datasets that exhibit distinct characteristics compared to the synthetic training data.

==> figures/fig_kitti-2.tex <==
\begin{figure}[htbp]
\vspace{-0.6cm} %%缩减间距
\setlength{\abovecaptionskip}{0cm}
\begin{center}
\begin{tabular}{@{}c@{} }
\includegraphics[width=0.45\textwidth, keepaspectratio]{figs/kitti_jz.png}
\put(-253,490){\rotatebox{90}{PointNorm-Net}}
\put(-253,360){\rotatebox{90}{DeepFit}}
\put(-253,205){\rotatebox{90}{NeuralGF}}
\put(-253,68){\rotatebox{90}{PCA}}
\end{tabular}
\end{center}
   \caption{PointNorm-Net identifies more geometry structures with higher quality on KITTI dataset. \jz{Colors encode the direction of normals. As shown in the coordinate system, the wall and sides of the vehicle should be green. The roof and hood of the car and ground should be blue. And the cars’ front facess hould be orange. Three car front faces are discovered by PointNorm-Net. While DeepFit, NeuralGF and PCA all failed to estimate faithful normals for the points on the cars’ front faces. NeuralGF even does not yield satisfactory results for the the sides of the vehicle.}
   }
\label{fig:KITTI-2}
\vspace{-0.8cm} %%缩减间距
\end{figure}

==> figures/tab_optimization_network_learning.tex <==
\begin{table*}[htbp]\small
\begin{center}
%\vspace{-0.3cm} %%缩减间距
\caption{\re{Evaluation of optimization and learning strategies within our multi-modal distribution estimation paradigm, using the PCPNet synthetic dataset. Opt-weight: PointNorm-Opt-weight, Opt-normal: PointNorm-Opt, PCPNet (ss): PointNorm-PCPNet, PCPNet (ms): PointNorm-Multi-PCPNet, DeepFit: PointNorm-Deepfit, \ie~ PointNorm-Net, Adafit: PointNorm-Adafit.} 
}
%\vspace{-0.3cm} %%缩减间距
\label{tab:optimization_network_learning}
%\resizebox{\columnwidth}{!}{
\begin{tabular}{p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
\hline
                &     \multicolumn{2}{c|}{Optimizing directly}   &    \multicolumn{2}{c|}{Point normal learning network} & \multicolumn{2}{c}{Point weight learning network}  \\
\hline
methods    &   Opt-weight & 	Opt-normal	& ~~PCPNet(ss)~~& 	PCPNet(ms)&	DeepFit& 	Adafit \\
\hline
RMS$\downarrow$ &  20.18&	14.86	&14.82	&14.36	&13.57	&12.36\\
\hline
\end{tabular}%}
%\vspace{-0.4cm} %%缩减间距
\end{center}
\end{table*}

==> supply.tex <==
\textbf{Validation of the proportion of candidates rejection.} In Section \ref{sec:Sel_candi_normasls}, we employ the idea of kernel density estimation to perform preliminary rejection of generated initial candidate normals. We observe that a larger rejection ratio does not necessarily yield better results during the {{filtering}} process, and there exists an optimal range for the rejection ratio. Here we have chosen to reject 10\% of  initial candidate normals. Excessively high rejection ratios can lead to a reduction in the number of sampled initial candidate normals, losing the accuracy of multi-sample consensus to a certain degree, as illustrated in \tab~\ref{tab:proportion_rejection}. 
\input{figures/tab_proportion_rejection}


\textbf{Validation of the adaptive neighborhood partition.} In Section \ref{sec:Optimization_NeighborSize}, the proposed algorithm adaptively determines the neighborhood size according to the noise scale of the point cloud.
%that is, the large noise uses a large neighborhood to sample points to generate initial candidate normals, and the small noise uses a small neighborhood. 
In experiments, we divide the neighborhood into four scales. We observe that the choice of dividing the neighborhood into 2, 3, or 4 segments did not have a significant impact on the experimental results, as shown in \tab~\ref{tab:neigh_seg}. Consequently, the 4-segments schedule is adopted based on the characteristics of the PCPNet dataset. Note that the model trained only on the PCPNet dataset with this option also performs well on the other three datasets as reported in the experiments above.
\input{figures/tab_NeighborSize}


\section{An implementation of the paradigm to self-supervised point cloud denoising}
\label{sec:extension}
The proposed multi-sample consensus paradigm is also applicable to other self-supervised tasks. This is shown by improving the cutting-edge self-supervised point cloud denoising method: DMR \cite{luo2020differentiable}. 
% Specifically, we follow the DMR denoising framework, only replacing its loss function and candidate sampling method. 
DMR follows the denoising loss defined in \cite{totaldenoise}:
\begin{equation}\label{eq:denoise_loss}
L_U=\frac{1}{N}\sum_{t=1}^{N}\sum_{\mathbf{q}}\|f(\mathbf{p}_t)-\mathbf{q}\|,
\end{equation}
%\begin{equation}\label{eq:denoise_loss}
%L_U=\frac{1}{N}\sum_{t=1}^{N}E_{q\sim P(q|p_t)}\|f(p_t)-q\|,
%\end{equation}
where $f(\cdot)$ represents the denoiser that maps a noisy point to a denoised point. Points $\{\mathbf{q}\}$ are sampled from the noisy
input point cloud $P$ according to a prior $P(\mathbf{q}|\mathbf{p}_t)$, which is empirically defined as: 
\begin{equation}
P(\mathbf{q}|\mathbf{p}_t)\propto exp(-\frac{\|\mathbf{q}-\mathbf{p}_t\|}{2\omega ^2}).
\end{equation}
Then the sampling point $\mathbf{q}$ is closer to the underlying clean surface with high probability.
However, it is not a suitable assumption for points around the sharp features. Although Hermosilla \etal~\cite{totaldenoise} employ RGB color annotation to overcome this problem, it only reduces it but does not eliminate it completely. Moreover, RGB color annotation is not always available.
The idea of {feasible candidate filtering} and {main mode estimation} can be employed to overcome this problem. Besides we design a novel sampling strategy to generate multiple and more accurate sampling points, $\{\mathbf{q}\}$, to guide the network training. 

\textbf{Candidate position initialization (CPI)}. Instead of sampling $\mathbf{q}$ from the input noisy point cloud $P$ directly, we first randomly select $k_s=4$ points in the $\hat{k}$ nearest neighbors of $\mathbf{p}_t$ and take their center as a candidate $\mathbf{q}$. This progress is repeated multiple times to obtain a set of candidates $\{\mathbf{q}\}$. $\hat{k}=64$ is the same as DMR.

\textbf{Feasible candidate filtering (FCF)}. A candidate is infeasible if there are fewer neighbors of $\mathbf{p}_t$ near it. Therefore, we compute a score for each candidate:
\begin{equation}
s^{t}_{\mathbf{q}}=\sum_{i=1}^{\hat{k}} e^{-\frac{\left(d(\mathbf{p}_{t}^{i},\mathbf{q})\right)^{2}}{\sigma^{2}}}, %\theta=1,2,\cdots,n
\end{equation}
where $\mathbf{p}_{t}^{i} \in \mathcal{N}_{\hat{k}}(\mathbf{p}_t)$ is a neighbor of $\mathbf{p}_{t}$, $d(\mathbf{p}_{t}^{i},\mathbf{q})$ represents the Euclidean distance from $\mathbf{p}_{t}^{i}$ to $\mathbf{q}$, and $\sigma$ is the bandwidth of the Gaussian kernel function. In the experiments, we set $\sigma$ to be equal to the average distance of the 12 nearest neighbor points of $\mathbf{p}_{t}$. Then the 10\% of initialized candidates with lower scores are deleted. 
%\jj{how many? or a threshold?}


\textbf{Main mode estimation}.  
A candidate consensus loss for position, similar with $L_{ccn}$, is defined as follows:
\begin{equation}
L_{ccp}=\sum_{\mathbf{q}}^{}-e^{-\frac{\left\|f(\mathbf{p}_{t}) - \mathbf{q}\right\|_{F}^{2}}{\tau^{2}}},
\end{equation}
where $\tau= \sigma$. 
It encourages the results to converge to the main mode supported by more inlier candidates.
%This results in convergence to the main mode supported by more inlier candidates. 

\input{figures/fig_denoise.tex}
\textbf{Dataset. }For training the denoising network, we have collected 13 different classes with 7 different meshes, each from ModelNet-40 \cite{modelnet-40}, and generate point clouds by randomly sampling 10K-50K points. The point clouds are then perturbed by Gaussian noise with standard deviations from 1\% to 3\% of the bounding box diagonal. Finally, a training dataset containing a total of 1365 models is generated. To be identical to the DMR training mechanism, we split the point cloud into patches consisting of 1024 points.
For testing, we have collected 20 classes with 3 meshes each. Similarly, we generate point clouds using randomly sampled 20K and 50K points, then perturb them by Gaussian noise with standard deviations of 1\%, 2\%, 2.5\%, and 3\% of the bounding box diagonal. Finally, a test dataset containing 480 models is generated.


\input{figures/tab_denoise.tex}
\textbf{Results. }We evaluate the effectiveness of our strategies quantitatively and qualitatively on the dataset.
For quantitative comparison, the Chamfer distance (CD) and point-to-surface distance (P2S) are used as evaluation metrics. As shown in \tab~\ref{tab:Denoising}, the CD and P2S are gradually improved by applying the three strategies. %\jj{what dataset?} with $\%1-3$ Gaussian noise. 
A qualitative comparison is also shown in \fig~\ref{fig:denoise}, where the colors encode the P2S errors.  Our results are much cleaner and exhibit more visually pleasing surfaces than those of DMR. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
